A Sensorimotor Reinforcement Learning Framework for Physical Human-Robot Interaction

Modeling of physical human-robot collaborations is generally a challenging problem due to the unpredictive nature of human behavior. To address this issue, we present a data-efficient reinforcement learning framework which enables a robot to learn how to collaborate with a human partner. The robot learns the task from its own sensorimotor experiences in an unsupervised manner. The uncertainty of the human actions is modeled using Gaussian processes (GP) to implement action-value functions. Optimal action selection given the uncertain GP model is ensured by Bayesian optimization. We apply the framework to a scenario in which a human and a PR2 robot jointly control the ball position on a plank based on vision and force/torque data. Our experimental results show the suitability of the proposed method in terms of fast and data-efficient model learning, optimal action selection under uncertainties and equal role sharing between the partners.

==> outline.tex <==
Outline of the paper:
% each number here means a paragraph
Introduction

1) Introducing pHRI 
2) What is the problem we are going to address
3) Why it is a challenging task
4) Leader/follower role assignment
5) Sensorimotor modeling and processing observation
6) Reinforcement learning
7) Structure of the paper

Related Work

1) robots with leader or follower roles
2) proactive behavior 
3) homotopy switching
4) impedance controller with equal role
5) our work

Methods

1) Short overview (SMC, Q) 
2) Outline of method section
3) Sensorimotor representation of the data
4) Data acquisition (need the training data to represent interaction parameters)
5) Forward model learning
6) GP regression

Method - Q Learning
1) Reinforcement / Q learning overview
2) Initialization of Q-function
3) Updating Q-function
4) Action selection based on Q 
5) UCB

Experiments

1) Setup
2) Forward model performance
3) Q function performance
4) Joint task compare two Q's
5) Joint task how is tau minimized


abstract: what do we do ( no motivation)

intro: future, middle: present, conclusion: past



